Mukayese: Turkish NLP Strikes Back

Having sufficient resources for language X lifts it from the under-resourced languages class, but not necessarily from the under-researched class. In this paper, we address the problem of the absence of organized benchmarks in the Turkish language. We demonstrate that languages such as Turkish are left behind the state-of-the-art in NLP applications. As a solution, we present Mukayese, a set of NLP benchmarks for the Turkish language that contains several NLP tasks. We work on one or more datasets for each benchmark and present two or more baselines. Moreover, we present four new benchmarking datasets in Turkish for language modeling, sentence segmentation, and spell checking. All datasets and baselines are available under: https://github.com/alisafaya/mukayese

==> dislaimer.tex <==

\textsc{\textbf{Update \ } It is a great pleasure to update my application with the fact that my paper has been accepted to appear in the \textbf{Findings of 60th Annual Meeting of the Association for Computational Linguistics (ACL) 2022}. The initial submission can be accessed via \href{https://openreview.net/forum?id=ThTMwcCPzkG}{\textcolor{blue}{this link}}. An updated submission which is likely to be more similar to the camera ready version can be accessed via \href{https://openreview.net/forum?id=l9H3-sPAnY}{\textcolor{blue}{this link}}. A deanonymized version of the paper is attached. }






==> sections/tasks/dependency-parsing.tex <==

% Arda
\subsection{Dependency parsing}
\label{subsec:dependency}

Dependency parsing focuses on the syntactic structure and the binary relation between words \cite{jurafsky-2018-speech}. In this binary relation, there is head and dependents. An example of such relation is shown in Figure \ref{fig:dep-tree}. In the Universal Dependencies (UD) Project \cite{nivre-etal-2016-universal}, set of binary relations for dependency parsing are introduced which can be applicable for different languages.

\begin{figure}[h]
\centering
\small
\begin{dependency}[edge horizontal padding=0]
\begin{deptext}
Bu, \& Rath'a \& göre \& tanrıçanın \& gücünü \& göstermektedir. \\
\end{deptext}
\depedge[edge unit distance=2ex]{6}{1}{nsubj}
\depedge{4}{3}{pobj}
\depedge[edge unit distance=2.5ex]{6}{3}{prep}
\depedge{5}{4}{poss}
\depedge{6}{5}{dobj}
\depedge{3}{2}{pobj}
\deproot{6}{root}
\end{dependency}
\caption{An example of dependency relations from Turkish Treebank Dataset \cite{kayadelen-etal-2020-LREC}.}
\label{fig:dep-tree}
\vspace{-5pt}
\end{figure}

% bedir-etal-2021-overcoming
% turk-etal-2019-turkish
% eryigit-etal-2011-multiword

%Syntactic Parsing.

%conll 2007 shared task: \cite{nivre-etal-2007-conll}
%conll 2018 shared task: \cite{zeman-etal-2018-conll}

\vspace{\subsubsectionspacing}
\textbf{Datasets \ \ }
In the dependency parsing benchmark, we use three different datasets. First dataset is UDBoun dataset \cite{turk-etal-2021-udboun}, which is also used in 2018 Conll task \cite{zeman-etal-2018-conll}. This dataset is collected from various resources including biographical texts, newspapers etc. The second dataset is METU-SABANCI treebank \cite{eryigit-etal-2011-multiword,oflazer-etal-2003-buildingtreebank,atalay-etal-2003-annotation}, and this dataset is used in 2007 CoNLL task \cite{nivre-etal-2007-conll}. The third dataset is Turkish Treebanks \cite{kayadelen-etal-2020-LREC}. This dataset includes two sections: first section is collected from forums and blogs; second section is collected from Wikipedia. This variety of datasets allowed us to build a benchmark including different domains.

%- https://github.com/UniversalDependencies/UD_Turkish-BOUN

%- https://web.itu.edu.tr/gulsenc/treebanks.html
% https://www.andrew.cmu.edu/user/ko/downloads/Papers/TurkishTreebank-Chapter.pdf

%- https://github.com/google-research-datasets/turkish-treebanks/

\vspace{\subsubsectionspacing}
\textbf{Evaluation \ \ }
Three different metrics are used for evaluating dependency parsing systems. Labeled Attachment Score (LAS) focuses on the dependency relations if both head and dependency relation in correctly detected. Morphology-Aware Labeled Attachment Score (MLAS) is similar to LAS but has more strict conditions for some relations. Bilexical dependency score (BLEX) metric is in agreement with the previous metrics, moreover this metric also focuses on the lemma of the word. The detailed descriptions of the metrics can be found at Conll task \cite{conll-2018-conll}.

%https://universaldependencies.org/conll18/evaluation.html

%- POS Tag accuracy
%- UAS -> Unlabeled attachment score
%- LAS -> Labeled attachment score
%- BLEX

%Evaluation script - https://universaldependencies.org/conll18/results.html

\vspace{\subsubsectionspacing}
\textbf{Baselines \ \ }
We used 2 different baselines for the task. First baseline is stanza \cite{qi-etal-2020-stanza}.
%- Stanza
%- https://github.com/google-research/turkish-morphology
%- https://arxiv.org/pdf/1908.07448v1.pdf
%- paperswithcode uzerinden en kolay train edilecek model

%https://paperswithcode.com/sota/dependency-parsing-on-penn-treebank


==> sections/tasks/morphological-analysis.tex <==
% Emirhan
\subsection{Morphological Analysis and Disambiguation}
\label{morphology}

The objective of morphological analysis is to generate all possible morphological parses for a given word. 

Even though a dictionary or a simple rule-based model is typically sufficient for morphologically simple languages \cite{minnen-etal-2001-applied}, for morphologically rich languages like Turkish \cite{oflazer-1993-two, oflazer-saraclar-2018-turkishnlp} more complex approaches are needed.

\vspace{\subsubsectionspacing}
\textbf{Datasets \ \ } In this task, we utilize two different datasets: \textsc{TrMor2018}  \cite{akyurek-etal-2019-morphological}, a manually annotated morphological analysis and disambugation dataset and \textsc{Turkish-BOUN} subset of \textsc{Universal Dependencies} \cite{turk-etal-2021-udboun}, a manually annotated treebank. As shown in in Table \ref{tab:morph-datasets}, \textsc{TrMor2018} is relatively 4 times bigger than \textsc{Turkish-BOUN}.

\begin{table}[ht]
	\centering
	\small
	\begin{tabular}{lllll}
		\toprule[1.5pt]
		& Train & Dev & Test & Total \\ \midrule
		\textsc{TRMor2018} & & & \\
		\#sentences           & 33K     & 722    & 776  &  35K \\
		\#words               &439K     & 10K    & 10K   &  459K    \\ \midrule
		\textsc{UD-BOUN} & & & \\
		\#sentences           & 7K     & 979     & 979  & 9K   \\
		\#words               & 98K     & 12K    & 12K     &  122K  \\ 
        \bottomrule[1.5pt]
	\end{tabular}
	\caption{Statistics of \textsc{TRMor2018} and \textsc{UD-BOUN} datasets' splits. \textsc{UD-BOUN} refers to Turkish-BOUN subset of Universal Dependencies Dataset.}
	\label{tab:morph-datasets}
	\vspace{-15pt}
\end{table}

\vspace{\subsubsectionspacing}
\textbf{Metrics \ \ } We measure the performance with accuracy, for whole-tag ignoring the lemma, and F1 Score based on the precision and recall of each morphological feature.

\vspace{\subsubsectionspacing}
\textbf{Baselines \ \ } For this problem, we train two different baselines, namely Morse \cite{akyurek-etal-2019-morphological}, an encoder-decoder model that does lemmatization and tagging simultaneously and Zemberek \cite{akin-dundar-2007-zemberek}, a rule-based analyser. Performances of our baselines are presented in \ref{tab:morph-results}. 

\begin{table}[ht]
	\centering
	\small
	\begin{tabular}{llll}
		\toprule[1.5pt]
		& F1 Score & Accuracy \\ \midrule
        \textsc{TRMor2018} & & \\
		Morse              & T       & T         \\
		Zemberek                & T        & T           \\
		\midrule
		\textsc{Y} & & \\
		Morse              & T       & T         \\
		Zemberek                & T        & T           \\
        \bottomrule[1.5pt]
	\end{tabular}
	\caption{Results of morphological disambiguation baselines}
	\label{tab:morph-results}
	\vspace{-15pt}
\end{table}



==> sections/tasks/question-answering.tex <==
\subsection{Question Answering}
\label{subsec:questionanswering}
